Image based Eye Gaze Tracking and its Applications

Eye movements play a vital role in perceiving the world. Eye gaze can give a direct indication of the users point of attention, which can be useful in improving human-computer interaction. Gaze estimation in a non-intrusive manner can make human-computer interaction more natural. Eye tracking can be used for several applications such as fatigue detection, biometric authentication, disease diagnosis, activity recognition, alertness level estimation, gaze-contingent display, human-computer interaction, etc. Even though eye-tracking technology has been around for many decades, it has not found much use in consumer applications. The main reasons are the high cost of eye tracking hardware and lack of consumer level applications. In this work, we attempt to address these two issues. In the first part of this work, image-based algorithms are developed for gaze tracking which includes a new two-stage iris center localization algorithm. We have developed a new algorithm which works in challenging conditions such as motion blur, glint, and varying illumination levels. A person independent gaze direction classification framework using a convolutional neural network is also developed which eliminates the requirement of user-specific calibration. In the second part of this work, we have developed two applications which can benefit from eye tracking data. A new framework for biometric identification based on eye movement parameters is developed. A framework for activity recognition, using gaze data from a head-mounted eye tracker is also developed. The information from gaze data, ego-motion, and visual features are integrated to classify the activities.

==> HeadTail/biodata.tex <==
\chapter*{Author's Biography}

\vspace*{0.15\textheight}

\textbf{{\em Anjith George}} is a Ph.D candidate from Department of Electrical 
Engineering, Indian Institute of Technology,
Kharagpur. He completed his B.Tech. degree in Electrical and Electronics Engineering
from NSS College of Engineering, University of Calicut during 2006-2010.  He completed his M. Tech in Instrumentation from IIT Kharagpur in 2012.  His research interests include Computer Vision, Pattern Recognition, Signal Processing, Gaze Tracking and it's applications.

 \subsection*{Contact Information}
 
Address: \= Thannikkapara House\\ Kolikkadavu, Payam P.O\\Kannur DT, Kerala\\PIN--670704\\India.
Mobile: +91-7501-549613 \\
Email: \href{mailto:anjith2006@gmail.com}{\nolinkurl{anjith2006@gmail.com}} \\
%LinkedIn: \url{https://www.linkedin.com/pub/anjith-george/29/25/874} \\



\subsection*{Research Interests} 
Human Computer Interaction, Gaze Tracking and applications, Biometrics, Computer Vision, Pattern Recognition and Machine Learning.

\subsection*{Education} 
\href{http://iitkgp.ac.in/}{\textbf {Indian Institute of Technology (IIT) }} Kharagpur, India. PhD (Ongoing), Image based Gaze tracking and Activity Recognition, July 2012- Current
                    
\href{http://iitkgp.ac.in/}{\textbf {Indian Institute of Technology (IIT) }} Kharagpur, India. M. Tech, Instrumentation Engineering, June 2012
                     
 
\href{http://www.nssce.ac.in/}{\textbf {N S S College of Engineering}}  \href{ http://www.universityofcalicut.info}{\textbf {(University of Calicut)}}, Kerala, India%http://www.nssce.ac.in/
 . B. Tech, Electrical and Electronics Engineering, June 2010

\textbf {St Mary's HSS Edoor}, Kerala, India. 12th 
 
\textbf {St Mary's HSS Edoor}, Kerala, India. 10th 

\subsection*{Awards \& Honours}
    \begin{itemize}  \itemsep -2pt % reduce space between items

                   \item \textbf{Winner}, BioEye 2015, International Eye Movement based biometrics competition, Organized by IEEE BTAS.
                  \item \textbf {Finalist}: Intel India Embedded Challenge 2012. 
                  \item \textbf{Secured 99.2 and 98.1 percentile} in Electrical engineering GATE 2010 and GATE 2012.
                  \item \textbf{MHRD Fellowship} during PhD (2012-Current)
                  \item \textbf{MHRD Fellowship} during M Tech (2010-2012)

                 \end{itemize}
                
\subsection*{Journal Publications} \begin{itemize}

\item \textbf{A. George}, A. Routray, ``Fast and Accurate Eye Localization Algorithm for Gaze Tracking in Low Resolution Images'', \textit{IET Computer Vision}, 2016.
\item \textbf{A. George}, A. Routray, ``A score level fusion method for eye movement biometrics'',
 \textit{Pattern Recognition Letters}, Elsevier, 2015.
\item A. Dasgupta, \textbf{A. George}, S. L. Happy, A. Routray, ``A Vision Based System for Monitoring the Loss of
Attention in Automotive Drivers'', in \textit{IEEE Transactions on Intelligent Transportation Systems}, vol. 14, no.
4, pp.1825-1838, 2013
\item A. Dasgupta, \textbf{A. George}, S. L. Happy, A. Routray, Tara Shanker, ``An on-board vision based system for
drowsiness detection in automotive drivers'', in \textit{International Journal of Advances in Engineering Sciences
and Applied Mathematics, Springer, Special Issue on Advanced Traffic and Transportation Systems}, vol. 5,
no. 2-3, pp. 94-103, 2013.

\end{itemize}             
\subsection*{Book Chapters} \begin{itemize}
\item A. Sengupta, \textbf{A. George}, A. Dasgupta, A. Chaudhuri, B. Kabi, A. Routray , ``Alertness monitoring system for vehicle drivers using physiological signals''. \textit{Handbook of Research on Emerging Innovations in Rail Transportation Engineering (\textbf{Book Chapter})}. IGI Global, 2016.

\end{itemize}  

\subsection*{Conference Publications} \begin{itemize}

\item \textbf{A. George}, A. Routray, ``Real-time Eye Gaze Direction Classification Using Convolutional Neural Network'', (Accepted), \textit{SPCOM, International Conference on Signal Processing and Communications, IEEE}, 2016.

\item A. Dasgupta, A. Mandloi, \textbf{A. George}, A. Routray, ``An Improved Algorithm for Eye Corner Detection'', (Accepted), \textit{SPCOM, International Conference on Signal Processing and Communications, IEEE }, 2016.

\item G. Banik, P. Patnaik, \textbf{A. George}, A. Routray, ``Contextual Priming and Perception Manipulation: An Exploration through Eye-Tracking and Audience Response'', \textit{ NAOP Convention 2016, Allahabad}.

\item SL Happy, A. Dasgupta, \textbf{A. George}, A. Routray, ``A video database of human faces under near Infra-Red illumination for human computer interaction applications'',
 \textit{ International Conference on Intelligent Human Computer Interaction (IHCI)}, IEEE, 2012.
 
\item SL Happy, \textbf{A. George}, A. Routray, ``A real time facial expression classification system using Local Binary Patterns'',
 \textit{ International Conference on Intelligent Human Computer Interaction (IHCI)}, IEEE, 2012.

\end{itemize}     

\subsection*{Patents} \begin{itemize}

\item ``A SYSTEM FOR REAL-TIME ASSESSMENT OF ALERTNESS LEVEL OF HUMAN BEINGS'', A. Routray, A. Dasgupta, \textbf{A. George}, SL Happy, 
 \textit{ 634/KOL/2013}, IN, 2013

\end{itemize}     





==> HeadTail/copyright.tex <==
\thispagestyle{empty}


\vskip 2.0\baselineskip \centerline{\Large{Indian Institute of
Technology}}

\begin{flushright}
{Date: February 2009}
\end{flushright}

Author: \bf{Anand S S} \\
Title: Techniques to Improve Information Extraction from Hyperspectral Remote Sensing Data\\
Department: Agricultural and Food Engineering\\
Degree: Ph.D\\
\vspace{0.5in} Permission is herewith granted to Indian Institute of
Technology, Kharagpur, India, to circulate and to have copied for
non-commercial purposes, at its discretion, the above title upon the
request of individuals or institutions.

\vspace{0.5in}

\begin{flushright}
Signature of Author
\end{flushright}
The author reserves other publication rights, and neither the thesis
nor extensive extracts from it may be printed or otherwise
reproduced without the author's written permission.


==> HeadTail/cv_anjith2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plasmati Graduate CV
% LaTeX Template
% Version 1.0 (24/3/13)
%
% This template has been downloaded from:
% http://www.LaTeXTemplates.com
%
% Original author:
% Alessandro Plasmati (alessandro.plasmati@gmail.com)
%
% License:
% CC BY-NC-SA 3.0 (http://creativecommons.org/licenses/by-nc-sa/3.0/)
%
% Important note:
% This template needs to be compiled with XeLaTeX.
% The main document font is called Fontin and can be downloaded for free
% from here: http://www.exljbris.com/fontin.html
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%----------------------------------------------------------------------------------------
%	PACKAGES AND OTHER DOCUMENT CONFIGURATIONS
%----------------------------------------------------------------------------------------

%\documentclass[a4paper,10pt]{article} % Default font size and paper size
%
%
%
%\usepackage[big]{layaureo} % Margin formatting of the A4 page, an alternative to layaureo can be \usepackage{fullpage}
%% To reduce the height of the top margin uncomment: \addtolength{\voffset}{-1.3cm}
%
%
%\usepackage{titlesec} % Used to customize the \section command
%\titleformat{\section}{\Large\scshape\raggedright}{}{0em}{}[\titlerule] % Text formatting of sections
%\titlespacing{\section}{0pt}{3pt}{3pt} % Spacing around sections

\vspace*{0.05cm}
\pagestyle{empty} % Removes page numbering
%\font\fb=''[cmr10]'' % Change the font of the \LaTeX command under the skills section
%----------------------------------------------------------------------------------------
%	NAME AND CONTACT INFORMATION
%----------------------------------------------------------------------------------------

\par{\centering{\Huge \bf ANJITH GEORGE}\bigskip\par} % Your name
\section{Contact details}
\begin{tabular}{rl}
\textsc{Permanent Address:} & Thannikkapara House, Kolikkadavu,\\& Payam P.O, Kannur DT, Kerala\\ &PIN--670704, India.\\

\textsc{Email:} & anjith2006@gmail.com\\
\textsc{Mobile:} & +91-7501-549613 \\

\end{tabular}
\section{Research Interests}
\begin{itemize}
  \item Computer vision
  \item Human computer interaction
  \item Gaze tracking and applications
  \item Pattern recognition and Machine learning
  \item Biometrics
  \item Deep learning
\end{itemize}


%%


%%
\section{Education}
\begin{tabular}{r|p{11cm}}
\textsc{2012-2016} &  \textbf{Ph.D Candidate}\\
& Image based eye gaze tracking and its applications\\
& Indian Institute of Technology Kharagpur, India\\
\multicolumn{2}{c}{} \\
%------------------------------------------------
\textsc{2010-2012} &  \textbf{M.Tech}\\
& Instrumentation Engineering\\
& Indian Institute of Technology Kharagpur, India\\
\multicolumn{2}{c}{} \\
%------------------------------------------------
\textsc{2006-2010} &  \textbf{B.Tech}\\
& Electrical and Electronics Engineering\\
& University of Calicut, Kerala, India\\
\end{tabular}
%----------------------------------------------------------------------------------------
%	WORK EXPERIENCE 
%----------------------------------------------------------------------------------------
\section{Awards \& Honours}
 \begin{itemize}  \itemsep -2pt % reduce space between items

                   \item \textbf{Winner}, BioEye 2015, International Eye Movement based biometrics competition, Organized by IEEE BTAS.
                  \item \textbf {Finalist}: Intel India Embedded Challenge 2012. 
                  \item \textbf{Secured 99.2 and 98.1 percentile} in Electrical engineering GATE 2010 and GATE 2012.
                  \item \textbf{MHRD Fellowship} during PhD (2012-Current)
                  \item \textbf{MHRD Fellowship} during M Tech (2010-2012)

                 \end{itemize}
\clearpage
\section{Publications}
\begin{itemize}

\item \textbf{A. George}, A. Routray, ``Fast and Accurate Eye Localization Algorithm for Gaze Tracking in Low Resolution Images'', \textit{IET Computer Vision},  (Available Online, DOI:  10.1049/iet-cvi.2015.0316), 2016.

\item \textbf{A. George}, A. Routray, ``A score level fusion method for eye movement biometrics'',
 \textit{Pattern Recognition Letters},  (Available Online, DOI:10.1016/j.patrec.2015.11.020), Elsevier, 2015.
\item A. Dasgupta, \textbf{A. George}, S. L. Happy, A. Routray, ``A Vision Based System for Monitoring the Loss of
Attention in Automotive Drivers'', in \textit{IEEE Transactions on Intelligent Transportation Systems}, vol. 14, no.
4, pp.1825-1838, 2013
\item A. Dasgupta, \textbf{A. George}, S. L. Happy, A. Routray, Tara Shanker, ``An on-board vision based system for
drowsiness detection in automotive drivers'', in \textit{International Journal of Advances in Engineering Sciences
and Applied Mathematics, Springer, Special Issue on Advanced Traffic and Transportation Systems}, vol. 5,
no. 2-3, pp. 94-103, 2013.

%\end{itemize}   
%\section{Book Chapters} \begin{itemize}
\item A. Sengupta, \textbf{A. George}, A. Dasgupta, A. Chaudhuri, B. Kabi, A. Routray , ``Alertness monitoring system for vehicle drivers using physiological signals''. \textit{Handbook of Research on Emerging Innovations in Rail Transportation Engineering}, pp. 273-311, IGI Global, 2016.
%\end{itemize}  

%\section{Conferences} \begin{itemize}

\item \textbf{A. George}, A. Routray, ``Real-time Eye Gaze Direction Classification Using Convolutional Neural Network'', (Accepted), \textit{SPCOM, International Conference on Signal Processing and Communications, IEEE}, 2016.

\item A. Dasgupta, A. Mandloi, \textbf{A. George}, A. Routray, ``An Improved Algorithm for Eye Corner Detection'', (Accepted), \textit{SPCOM, International Conference on Signal Processing and Communications, IEEE }, 2016.

\item G. Banik, P. Patnaik, \textbf{A. George}, A. Routray, ``Contextual Priming and Perception Manipulation: An Exploration through Eye-Tracking and Audience Response'', \textit{ NAOP Convention 2016, Allahabad}.

\item SL Happy, A. Dasgupta, \textbf{A. George}, A. Routray, ``A video database of human faces under near Infra-Red illumination for human computer interaction applications'',
 \textit{ International Conference on Intelligent Human Computer Interaction (IHCI)}, IEEE, 2012.
 
\item SL Happy, \textbf{A. George}, A. Routray, ``A real time facial expression classification system using Local Binary Patterns'',
 \textit{ International Conference on Intelligent Human Computer Interaction (IHCI)}, IEEE, 2012.

\end{itemize}     

\section{Patents} \begin{itemize}

\item ``A SYSTEM FOR REAL-TIME ASSESSMENT OF ALERTNESS LEVEL OF HUMAN BEINGS'', A. Routray, A. Dasgupta, \textbf{A. George}, SL Happy, 
 \textit{ 634/KOL/2013}, IN, 2013

\end{itemize}     


\rule{410pt}{2pt}



==> Makefile <==
# Created by Andre Anjos <andre.anjos@idiap.ch>
# Tue 18 Apr 2017 11:50:17 CEST

# Builds the LaTeX project as a PDF document

TEXFILE=main.tex
PDFFILE=$(TEXFILE:%.tex=%.pdf)

%.pdf: %.tex
	pdflatex $(@:%.pdf=%.tex); \
	bibtex $(@:%.pdf=%); \
	pdflatex $(@:%.pdf=%.tex); \
	pdflatex $(@:%.pdf=%.tex);

all: $(PDFFILE)

.PHONY: clean

clean:
	@rm -vf $(shell find . -name "*~")
	@rm -vf *.log *.lot *.lof *.loa *.toc *.idx *.inc *.ilg *.ind *.blg
	@rm -vf *.aux *.glo *.dvi *.ps main.pdf *.out *.brf $(PDFFILE)
